Active Visual Localization for Multi-Agent Collaboration: A Data-Driven Approach

Rather than having each newly deployed robot create its own map of its surroundings, the growing availability of SLAM-enabled devices provides the option of simply localizing in a map of another robot or device. In cases such as multi-robot or human-robot collaboration, localizing all agents in the same map is even necessary. However, localizing e.g. a ground robot in the map of a drone or head-mounted MR headset presents unique challenges due to viewpoint changes. This work investigates how active visual localization can be used to overcome such challenges of viewpoint changes. Specifically, we focus on the problem of selecting the optimal viewpoint at a given location. We compare existing approaches in the literature with additional proposed baselines and propose a novel data-driven approach. The result demonstrates the superior performance of the data-driven approach when compared to existing methods, both in controlled simulation experiments and real-world deployment.

==> chapters/abstract.tex <==
\chapter*{Abstract}
\addcontentsline{toc}{chapter}{Abstract}

Robotic autonomy in complex indoor environments relies on accurate mapping. Multi-agent approaches to the problem of efficient map generation, where data collected with devices such as Mixed-Reality headsets is utilized, can make robot localization challenging due to occlusions and large viewpoint changes. This work focuses on tackling this localization challenge by using an Active Vision system to make informed viewpoint selections for a ground robot within point-cloud maps generated from data recorded from a Mixed-Reality headset.

A variety of viewpoint selection methods were evaluated and a novel data-driven approach to the problem was explored. By making use of simulated environments and data-collection methods, this work manages to overcome some limitations of real-world hardware, allowing for an extensive evaluation of different methods. The novel data-driven methods, especially the VPT (Viewpoint Transformer), show promising results, given their capability to incorporate different types of landmark information in a per-landmark fashion. This potential is further highlighted by the performance when deployed in a real-world setting on the  Boston Dynamics Spot quadruped robot.

This work also shows the importance of occlusion information in multi-agent localization scenarios. Methods that consider landmark viewing direction during the mapping process are able to overcome some occlusion issues by selecting viewpoints that are more similar to those used to map the environment, making them especially relevant when only image data is available.

While the results are promising, differences between simulated and real-world experiments suggest further development and evaluation is still required. However, this work highlights the potential of Active Vision and data-driven methods in improving ground-robot localization in multi-agent mapping settings.

==> chapters/chapter.tex <==
\chapter{Einige wichtige Hinweise zum Arbeiten mit \LaTeX\ }
\label{sec:latexumg}

Nachfolgend wird die Codierung einiger oft verwendeten Elemente
kurz beschrieben. Das Einbinden von Bildern ist in \LaTeX\ nicht
ganz unproblematisch und hängt auch stark vom verwendeten Compiler
ab. Typisches Format für Bilder in \LaTeX\ ist
EPS\footnote{Encapsulated Postscript} oder PDF\footnote{Portable Document Format}.


\section{Gliederungen}
\label{sec:gliederung}

Ein Text kann mit den Befehlen \texttt{\textbackslash
chapter\{.\}}, \texttt{\textbackslash section\{.\}},
\texttt{\textbackslash subsection\{.\}} und \texttt{\textbackslash
subsubsection\{.\}} gegliedert werden.


\section{Referenzen und Verweise}
\label{sec:refverw}

Literaturreferenzen werden mit dem Befehl \texttt{\textbackslash
citep\{.\}} und \texttt{\textbackslash
citet\{.\}} erzeugt. Beispiele: ein Buch \citep{Raibert1986LeggedRobotsThatBalance}, ein Buch und ein Journal Paper \citep{Raibert1986LeggedRobotsThatBalance,Vukobratovic2004ZeroMomentPoint}, ein Konferenz Paper mit Erwähnung des Autors: \citet{Pratt1995SEA}.

Zur Erzeugung von Fussnoten wird der Befehl \texttt{\textbackslash
footnote\{.\}} verwendet. Auch hier ein Beispiel\footnote{Bla
bla.}.

Querverweise im Text werden mit \texttt{\textbackslash label\{.\}}
verankert und mit \texttt{\textbackslash cref\{.\}} erzeugt.
Beispiel einer Referenz auf das zweite Kapitel:
\cref{sec:latexumg}.


\section{Aufzählungen}\label{sec:aufz}

Folgendes Beispiel einer Aufzählung ohne Numerierung,
\begin{itemize}
  \item Punkt 1
  \item Punkt 2
\end{itemize}
wurde erzeugt mit:
\begin{verbatim}
\begin{itemize}
  \item Punkt 1
  \item Punkt 2
\end{itemize}
\end{verbatim}

Folgendes Beispiel einer Aufzählung mit Numerierung,
\begin{enumerate}
  \item Punkt 1
  \item Punkt 2
\end{enumerate}
wurde erzeugt mit:
\begin{verbatim}
\begin{enumerate}
  \item Punkt 1
  \item Punkt 2
\end{enumerate}
\end{verbatim}

Folgendes Beispiel einer Auflistung,
\begin{description}
  \item[P1] Punkt 1
  \item[P2] Punkt 2
\end{description}
wurde erzeugt mit:
\begin{verbatim}
\begin{description}
  \item[P1] Punkt 1
  \item[P2] Punkt 2
\end{description}
\end{verbatim}


\section{Erstellen einer Tabelle}\label{sec:tabellen}

Ein Beispiel einer Tabelle:
\begin{table}[h]
\begin{center}
 \caption{Daten der Fahrzyklen ECE, EUDC, NEFZ.}\vspace{1ex}
 \label{tab:tabnefz}
 \begin{tabular}{ll|ccc}
 \hline
 Kennzahl & Einheit & ECE & EUDC & NEFZ \\ \hline \hline
 Dauer & s & 780 & 400 & 1180 \\
 Distanz & km & 4.052 & 6.955 & 11.007 \\
 Durchschnittsgeschwindigkeit & km/h & 18.7 &  62.6 & 33.6 \\
 Leerlaufanteil & \% & 36 & 10 & 27 \\
 \hline
 \end{tabular}
\end{center}
\end{table}

Die Tabelle wurde erzeugt mit:
\begin{verbatim}
\begin{table}[h]
\begin{center}
 \caption{Daten der Fahrzyklen ECE, EUDC, NEFZ.}\vspace{1ex}
 \label{tab:tabnefz}
 \begin{tabular}{ll|ccc}
 \hline
 Kennzahl & Einheit & ECE & EUDC & NEFZ \\ \hline \hline
 Dauer & s & 780 & 400 & 1180 \\
 Distanz & km & 4.052 & 6.955 & 11.007 \\
 Durchschnittsgeschwindigkeit & km/h & 18.7 &  62.6 & 33.6 \\
 Leerlaufanteil & \% & 36 & 10 & 27 \\
 \hline
 \end{tabular}
\end{center}
\end{table}
\end{verbatim}


\section{Einbinden einer Grafik}\label{sec:epsgraph}

Das Einbinden von Graphiken kann wie folgt bewerkstelligt werden:
\begin{verbatim}
\begin{figure}
   \centering
   \includegraphics[width=0.75\textwidth]{images/k_surf.pdf}
   \caption{Ein Bild.}
   \label{fig:k_surf}
\end{figure}
\end{verbatim}

\begin{figure}
   \centering
   \includegraphics[width=0.75\textwidth]{images/k_surf.pdf}
   \caption{Ein Bild}
   \label{pics:k_surf}
\end{figure}

oder bei zwei Bildern nebeneinander mit:
\begin{verbatim}
\begin{figure}
  \begin{minipage}[t]{0.48\textwidth}
    \includegraphics[width = \textwidth]{images/cycle_we.pdf}
  \end{minipage}
  \hfill
  \begin{minipage}[t]{0.48\textwidth}
    \includegraphics[width = \textwidth]{images/cycle_ml.pdf}
  \end{minipage}
  \caption{Zwei Bilder nebeneinander.}
  \label{pics:cycle}
\end{figure}
\end{verbatim}

\begin{figure}
  \begin{minipage}[t]{0.48\textwidth}
    \includegraphics[width = \textwidth]{images/cycle_we.pdf}
  \end{minipage}
  \hfill
  \begin{minipage}[t]{0.48\textwidth}
    \includegraphics[width = \textwidth]{images/cycle_ml.pdf}
  \end{minipage}
  \caption{Zwei Bilder nebeneinander}
  \label{pics:cycle}
\end{figure}


\section{Mathematische Formeln}\label{sec:math}

Einfache mathematische Formeln werden mit der equation-Umgebung
erzeugt:
\begin{equation}
 p_{me0f}(T_e,\omega_e) \ = \ k_1(T_e) \cdot (k_2+k_3 S^2
 \omega_e^2) \cdot \Pi_{\mathrm{max}} \cdot \sqrt{\frac{k_4}{B}} \, .
 	\label{eq:my_equation}
\end{equation}

Der Code dazu lautet:
\begin{verbatim}
\begin{equation}
 p_{me0f}(T_e,\omega_e) \ = \ k_1(T_e) \cdot (k_2+k_3 S^2
 \omega_e^2) \cdot \Pi_{max} \cdot \sqrt{\frac{k_4}{B}} \, .
\end{equation}
\end{verbatim}

Mathematische Ausdrücke im Text werden mit \$formel\$ erzeugt (z.B.:
$a^2+b^2=c^2$).

Vektoren und Matrizen werden mit den Befehlen \texttt{\textbackslash vec\{.\}} und \texttt{\textbackslash mat\{.\}} erzeugt (z.B. $\vec{v}$, $\mat{M}$).


\section{Weitere nützliche Befehle}\label{sec:div}

Hervorhebungen im Text sehen so aus: \emph{hervorgehoben}. Erzeugt
werden sie mit dem \texttt{\textbackslash epmh\{.\}} Befehl.

Einheiten werden mit den Befehlen \texttt{\textbackslash unit[1]\{m\}} (z.B.~\unit[1]{m}) und \texttt{\textbackslash unitfrac[1]\{m\}\{s\}} (z.B.~\unitfrac[1]{m}{s}) gesetzt.


==> chapters/discussion.tex <==
\chapter{Discussion}

\section{Viewpoint Strategy Evaluation - Simulation}
When considering the results from the simulated environments, it is evident that active viewpoint-choosing strategies outperform the baseline methods in many cases. While the evaluation within the simulated environment only explores a limited range of all variables that can affect the mapping and localization process, it shows the potential of being able to generate large amounts of data from varying scenarios and enabling the structured evaluation of methods that are otherwise hard to quantify when using real-world hardware and datasets. A study of this kind where 4 different indoor environments are evaluated at over 2000 unique data points would be prohibitively difficult to achieve outside of simulation, especially when considering the 25000 unique data points collected from a further five environments in order to train the data-driven approaches. 

\subsection{Data-Driven Approaches}
In the maps of simulated environments created with the same local feature type which was used to train the data-driven approaches, the results show that learning the decision boundaries of landmark features and the ability to include a variety of different information allows the methods to outperform the tested methods that use hand-crafted information metrics. This indicates the potential such data-driven approaches have by taking a less heuristic approach to the problem.
While the performance margins within the experiments are relatively small, it is promising that the methods were able to learn strategies at least as good as those hand-crafted or based on information theory, such as \textit{FIM}. Even if this potential was not fully exploited in this work, it points to the fact that perhaps with other features or information formulation, there is still room for improvement, especially when considering the comparison to the \textit{Best Possible} localization results.


\subsubsection{AVFN vs. VPT}
When considering the two types of data-driven methods evaluated for this work, the results offer some insight into the differences between them. Despite the fact that the methods were trained using the same learning objective and loss function, the differing performance in the evaluated experiments suggests that approaches did in fact learn at least slightly different methods due to their different architectures. While the performance differences between them are small in some evaluation scenarios, they become more significant in others, such as when the models are trained without considering occlusion or with changes in map representation.

While the \textit{VPT} and \textit{AVFN} both use largely the same input information, the ability of the \textit{VPT} to include information in a per-landmark fashion enables other types of information to be used. While not all evaluation scenarios show differences, the improved \textit{VPT} performance in the SIFT maps when including DINO features may suggest that the ability to add other types of information has further unexplored potential. The large performance difference between the two data-driven methods in the real-world evaluation could also hint at potentially better generalization capabilities of the \textit{VPT}.

\subsubsection{DINO Features}
DINO features were added as input to the \textit{VPT} network as a method of including coarse landmark appearance information. While the generalization results in SIFT maps suggest that they do have at least some influence on the \textit{VPT} decisions when choosing viewpoints, the results in the other experiments do not conclusively suggest that DINO is a viable way of including appearance information as input for viewpoint decisions.

A plausible explanation could be that appearance features do not offer clear information when it comes to the very general task of indoor localization, where environment appearance can vary greatly. Scenarios studied in work such as \cite{Bartolomei2021Semantic-awareLearning} often have a clear correlation between appearance and localization utility, whereas the diversity of indoor environments may make drawing generalizations of appearance information more difficult.

\subsubsection{Generalization}
The significant performance variation when shifting from SuperPoint to SIFT features, and then further from simulation to real-world deployment, underscores the challenges in generalizing viewpoint strategies across different feature descriptors and environments. The methods' inability to consistently retain their relative performance rankings indicates that while certain approaches might excel in specific settings, there may not be a one-size-fits-all solution.

However, the fact that in all three evaluated scenarios, a data-driven approach performed best across most thresholds, may suggest that these approaches offer the most potential for a generalizable solution to the problem of viewpoint selection. This would of course require a much larger dataset and diverse training environments to fully investigate.

\subsection{Occlusion}
Across different maps and methods, it is clear to see that methods that consider landmark occlusion perform significantly better than those that do not. While this may be obvious, it is worth examining how strongly occlusion affects certain types of methods compared to others. This is especially relevant when considering that environments in which robots are deployed may not have been mapped with devices that provide the necessary depth data to perform an accurate mesh reconstruction. For instance, one could imagine a robot deployment in a public indoor space where many images are available online. While the images could be used to create an initial map for robot navigation, landmark occlusion during the mission would be hard to determine without a full mesh reconstruction. 
However, when comparing the performance of methods that utilize occlusion information versus those that do not, it becomes clear that methods that consider the direction from which landmarks were viewed fare noticeably better, for example when compared to the large performance drop-off of the \textit{Maximum Criteria}. An explanation for this could be that choosing the viewpoint with the maximum number of landmarks that were viewed from a similar direction inherently leads to choosing viewpoints that are similar to those used to map the environment. This similarity then improves all steps of the localization pipeline, leading to better image retrieval using the global images feature and more numerous and robust local feature matches.

The fact that the \textit{VPT} was able to perform better than the \textit{Angle Criteria (occ.)} in the experiment shown in Table \ref{tab:SP_results} also suggests that data-driven approaches with a transformer architecture are capable of handling the scenario where no occlusion information is available by incorporating other landmark information than just viewing direction, or perhaps even learn a coarse occlusion estimate from the landmark features.

\section{Quadruped Deployment}
The deployment of the investigated methods on a real quadruped robot primarily serves as validation that the methods developed in simulation transfer to real hardware and mapping scenarios. Overall, the results on the Boston Dynamics Spot robot indicate that, while there are noticeable differences in the performance in the simulation environments, the methods developed in simulation show signs of improved localization capabilities in the real world, with active viewpoint-choosing strategies outperforming baseline methods in the majority of cases.

While the \textit{VPT} showed the best performance in the real-world evaluations, it is hard to draw definitive conclusions from the experiment. As discussed in Section \ref{sec:spot_exp_eval}, the localization performance in this scenario is not easy to measure. While the chosen method of measuring the robot body location using a combination of the map and fiducial markers provides a good estimate, more extensive testing could be conducted with a more accurate measurement setup. 

In addition, the small sample size of the experiment consisting of 12 locations in the environment, is most likely insufficient to draw conclusions with as much certainty as from the simulated experiments.

The differences in performance compared to the simulation experiments could be the result of many factors. As opposed to the simulated environments, the real-world scenario introduces many variables not modelled in the simulation. For instance, the simulated experiments use environments that stay exactly the same during the mapping process and the localization, whereas small changes in the environment are inevitable in the real world. An approach to closing this gap would be to vary the situations used in the simulation by modelling additional variables, such as lighting or non-static obstacles, such as humans moving around during the mapping process, or furniture being moved between mapping and later localization. It is also worth noting that the evaluations with the real robot were conducted at different mapping and robot heights than in the simulation.

Despite this sim-to-real gap, the \textit{VPT} still manages to perform across both scenarios, perhaps hinting further at the capabilities of the network to generalize across these changing scenarios.




==> chapters/preface.tex <==
\chapter*{Preface}
\addcontentsline{toc}{chapter}{Preface}
%\chapter*{Vorwort}
%\addcontentsline{toc}{chapter}{Vorwort}
This report summarizes the work done during my Master Thesis and marks the final step on my journey towards a Master's degree in Robotics, Systems and Control at ETH Zurich.

I would like to express my gratitude to Dr. Hermann Blum and Boyang Sun for providing guidance and support throughout the project.
